Fluorescence enabled phonon counting in an erbium doped piezo-optomechanical microcavity

Converting phonons to photons with optomechanical interaction provides a pathway to realize single phonon counting, which is instrumental in the quantum applications of mechanical systems such as entanglement generation, thermometry, and study of macroscopic quantum phenomenon. In this process, the key requirement is high-extinction, narrowbandwidth, and stable filtering of the parametric optical pump. Here, we propose to lift this necessity by counting fluorescence emission from a rare earth embedded optomechanical cavity. By doing so, we show that an equivalent filtering effect can be achieved due to spectral hole burning and cavity Purcell effect. To demonstrate this, we designed, fabricated, and characterized an integrated piezo-optomechanical FabryPerot cavity on the erbium doped thin-film lithium niobate platform. By collecting fluorescence from the optomechanical sideband, we show that 93dB suppression of the pump can be achieved with 10dB loss of signal, resulting in an increase of 83dB in sidebandpump ratio. Our results facilitate a route to realize f ilterless single phonon counting and also create new opportunities to study the interaction between solid state emitters and mechanical systems.

==> README <==
                 The dgruyter package:                 
preparing books and journals for Walter de Gruyter GmbH


File:       README
Author:     le-tex publishing services


DESCRIPTION
===========

The dgruyter package assists in preparing manuscripts for de Gruyter
with {\LaTeX}. It provides some special commands for journal papers
as well as for books and generates the required appearance.
Together with corresponding font packages it allows to produce the 
final layout of De Gruyter books and journal articles.

Copyright:  (C) 2015--2022 Walter de Gruyter GmbH


FILES IN DISTRIBUTION
=====================

   BASE DISTRIBUTION:

      README                  This file.
      dgruyter.ins            Package installation file.
      dgruyter.dtx            Package source file.
      dg-degruyter.eps/.pdf   Logo files.
      dg-mouton.eps/.pdf      Logo files.
      dg-saur.eps/.pdf        Logo files.
      DG_attention.eps/.pdf   Vignette files.
      DG_exercise.eps/.pdf    Vignette files.
      DG_information.eps/.pdf Vignette files.
      DG_notice.eps/.pdf      Vignette files.
      DG_question.eps/.pdf    Vignette files.
      book.tex                Template file for a book.
      article.tex             Template file for a journal article.

   DOCUMENTATION:

      dgruyter.pdf            User manual for dgruyter package. 
                              It is produced as described below.


BASIC INSTALLATION
====================

   To get the package style file 'dgruyter.sty' and the
   index style files 'dgruyter.ist' and 'dgruyter.xdy' execute:
     latex dgruyter.ins

   The minimum requirement to use the package is to have
     dgruyter.sty and dgruyter.ist/dgruyter.xdy
     (as well as the logo and vignette files)
     in a directory where TeX can find it.

   To get the documentation 'dgruyter.pdf' execute:
     pdflatex dgruyter.dtx (at least twice)

